High order recovery of geometric interfaces from cell-average data

We consider the problem of recovering characteristic functions $u:=\chi_\Omega$ from cell-average data on a coarse grid, and where $\Omega$ is a compact set of $\mathbb{R}^d$. This task arises in very different contexts such as image processing, inverse problems, and the accurate treatment of interfaces in finite volume schemes. While linear recovery methods are known to perform poorly, nonlinear strategies based on local reconstructions of the jump interface $\Gamma:=\partial\Omega$ by geometrically simpler interfaces may offer significant improvements. We study two main families of local reconstruction schemes, the first one based on nonlinear least-squares fitting, the second one based on the explicit computation of a polynomial-shaped curve fitting the data, which yields simpler numerical computations and high order geometric fitting. For each of them, we derive a general theoretical framework which allows us to control the recovery error by the error of best approximation up to a fixed multiplicative constant. Numerical tests in 2d illustrate the expected approximation order of these strategies. Several extensions are discussed, in particular the treatment of piecewise smooth interfaces with corners.

==> configuration.tex <==
\usepackage[utf8]{inputenc}

\usepackage{amsmath}
\usepackage{amssymb}  % for mathbb

\usepackage{varioref}       
\usepackage[hidelinks]{hyperref} % for clickable references inside document. [hidelinks] to avoid red boxes in clickable links.
\usepackage{cleveref}   

\usepackage{caption}
\usepackage{subcaption}
\usepackage{graphicx}  % include images
\usepackage{placeins}  % for FloatBarrier
\usepackage{grffile}
\usepackage[usenames,dvipsnames]{xcolor}  % for colors; for named colors: https://steeven9.github.io/USI-LaTeX/html/packages_hyperref_babel_xcolor3.html
\usepackage{listings} % to include code blocks
\usepackage{xcolor}
% \usepackage[pdftex,dvipsnames]{xcolor}  % Coloured text etc.
\usepackage{tabularray} % tblr 

\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{calc}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                       Comments                           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{xargs} % Use more than one optional parameter in a new commands
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\info}[2][1=]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,#1]{#2}}
\newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                       Colors                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                  Algorithms style                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}

% Marking commands: DONE etc.
\newcommand{\colored}[2]{{\color{#1}{#2}}}
\newcommand{\problems}[0]{{\color{red}{\textbf{Problems }}}}
\newcommand{\questions}[0]{{\color{red}{\textbf{Questions }}}}
\newcommand{\done}[0]{{\color{ForestGreen}{\textbf{Done }}}}
\newcommand{\codedone}[0]{{\color{ForestGreen}{\textbf{Code done }}}}
\newcommand{\written}[0]{{\color{ForestGreen}{\textbf{Written }}}}
\newcommand{\progress}[0]{{\color{Dandelion}{\textbf{In progress }}}}
\newcommand{\codeprogress}[0]{{\color{Dandelion}{\textbf{Code in progress }}}}
\newcommand{\writing}[0]{{\color{Dandelion}{\textbf{Writing }}}}


\newcommand{\towrite}[1]{{\color{NavyBlue}{\textbf{To write} #1}}}
\newcommand{\question}[1]{{\color{BrickRed}{\textbf{To write} #1}}}
\newcommand{\comment}[1]{{\color{ForestGreen}{\textbf{To write} #1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                  Common notation                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Variables for text formatting
\newcommand{\FamiliesScale}{0.2}

\newcommand\eps{\varepsilon}
\newcommand\e{\varepsilon}
\newcommand\dist{\text{dist}}
\newcommand\diff{\text{diff}}
\renewcommand\t{\tilde}
\newcommand\wt{\widetilde}
\newcommand\<{\langle}
\renewcommand\>{\rangle}
\renewcommand\leq{\leqslant}
\renewcommand\geq{\geqslant}

% \newenvironment{disarray}{\everymath{\displaystyle\everymath{}}\array}{\endarray}
% \def\cM{{\cal M}}
% \def\cN{{\cal N}}
% \def\cP{{\cal P}}
% \def\cT{{\cal T}}
% \def\cB{{\cal B}}
% \def\cF{{\cal F}}
% \def\cC{{\cal C}}
% \def\cL{{\cal L}}
% \def\cK{{\cal K}}
% \def\bj{{\bf j}}
% \def\bl{{\bf \ell}}
% \def\o{\overline}
% \def\nl{\newline}
% \def\vp{\varphi}
% \def\({\left (}
% \def\){\right )}

\newcommand{\R}{\mathbb R}
\newcommand{\N}{\mathbb N}
\newcommand{\Pp}{\mathbb P}
\def\Chi{\raise .3ex\hbox{\large $\chi$}}
% \renewcommand{\theequation}{\thesection.\arabic{equation}}
% \newcommand{\be}{\begin{equation}}
% \newcommand{\ee}{\end{equation}}
% \newcommand{\iref}[1]{{\rm (\ref{#1})}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}

% \DeclareMathOperator{\supp}{supp}
% \DeclareMathOperator{\divergence}{div}
% \DeclareMathOperator{\id}{id}
% \DeclareMathOperator{\argmin}{argmin}
% \DeclareMathOperator{\Span}{span}

\newcommand{\twopartdef}[4]
{
	\left\{
		\begin{array}{ll}
			#1 & \mbox{if } #2 \\
			#3 & \mbox{if } #4
		\end{array}
	\right.
}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\ud}{\,\mathrm{d}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                       Notation                           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\f}{u} % function
\newcommand{\fapprox}{\t \f} % function approximation

\newcommand{\cellavg}{a} % avg cells
\newcommand{\curve}{\gamma} % curve
\newcommand{\curveparams}{\theta} % curve parameters
\newcommand{\neigh}{\mathcal{N}} % curve parameters



\newcommand{\avgcc}{\cellavg_{CC}}
\newcommand{\avgccapprox}{\t \avgcc}
\newcommand{\avgnorm}{X}
\newcommand{\onedavgnorm}{Y}
\newcommand{\cellavgapprox}{\t \cellavg}
\newcommand{\flux}{\mathcal F}

\newcommand{\onedtransform}{g}
\newcommand{\aeroexplicit}{A}

\newcommand{\cellonedavg}{v}


% local approximation
\newcommand{\localf}{f_{\Omega}}
\newcommand{\localfparams}{\localf_{\curveparams}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                      Tikz figures                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{gridcolor}{RGB}{192, 192, 192} % Gray color for grid
\definecolor{domaincolor}{RGB}{34, 139, 34} % Forest green color for domain

% Define the new command \zoomedInFigure
\newcommand{\zoomedInFigure}[3]{
% \coordinate (O) at $#1*(-#2, -#3)$;
  % \begin{scope}[shift={O}, scale=#1]
  \begin{scope}[shift={(-#2*#1,-#3*#1)}, scale=#1]
    % Define the translated and scaled coordinates for the smooth domain
    \coordinate (A) at (3,2.5);
    \coordinate (B) at (4,8);
    \coordinate (C) at (7.7,7);
    \coordinate (D) at (6.3,2);
    \coordinate (E) at (3,2.5);
    
    % Draw the zoomed-in smooth domain
    \draw[thick, smooth cycle, tension=0.4, color=domaincolor, fill=domaincolor!30] 
      (A) to[out=90,in=180] (B) to[out=0,in=90] (C) 
      to[out=270,in=0] (D) to[out=180,in=270] (E);
  \end{scope}
}


\newcommand{\PlotSubCellDiagramDD}{

    \def\zoom{2}
    \def\cellx{7}
    \def\celly{6}
\begin{tikzpicture}[scale=0.6]
  % Draw the smooth domain
  \zoomedInFigure{1}{0}{0}

  % Draw the grid
  \draw[step=1, line width=0.2mm, color=gridcolor] (0,0) grid (10,10);

  % Add label for the domain
  \node[below, color=domaincolor] at (5,5) {$\Omega$};
  
  % Draw h
  \draw[-, line width=0.2mm] (2,11) -- (3,11);
  \node[right] at (1.75,12) {$h$};
  
  % draw approximation
  \begin{scope}
    \clip (\cellx-1, \celly-1) rectangle (\cellx+2, \celly+2);
    \draw[blue, dashed, thick] plot [domain={\cellx-1}:{\cellx+1}] (\x,{0.5+\celly - 6*(\x-0.75-\cellx)});
  \end{scope}
  \begin{scope}
    \clip (\cellx, \celly) rectangle (\cellx+1, \celly+1);
    \draw[blue, thick] plot [domain={\cellx-1}:{\cellx+1}] (\x,{0.5+\celly - 6*(\x-0.75-\cellx)});
  \end{scope}
    
  % Neighborhood
  \draw[black, dotted, line width=0.3mm] (\cellx-1,\celly-1) rectangle (\cellx+2,\celly+2);
  \node[right] at (\cellx-0.25,\celly+3) {$\mathcal{N}_{ij}$};

  % Mark a specific grid cell with a red square
  \draw[red, line width=0.3mm] (\cellx,\celly) rectangle (\cellx+1,\celly+1);
  \node[right, red] at (\cellx-2.75,\celly+0.5) {$C_{ij}$};
  
  % Zoomed-in view
  \begin{scope}[shift={(12,2)}]
    % Draw the zoomed-in plot
    \clip (0, 0) rectangle (\zoom*3, \zoom*3);
    \fill[fill=blue!30, opacity=0.75] (0, 0) -- plot [domain=\zoom*0:\zoom*3] (\x,{1.5*\zoom - 2*\zoom*(\x-1.75*\zoom)}) -- cycle;
    \zoomedInFigure{\zoom}{6}{5};
    % draw grid
    \draw[step=\zoom, line width=0.3mm, color=gridcolor] (0,0) grid (\zoom*3,\zoom*3);
    % draw line
    \draw[blue, dashed, thick] plot [domain=\zoom*0:\zoom*3] (\x,{1.5*\zoom - 2*\zoom*(\x-1.75*\zoom)});
    \begin{scope}
        \clip (\zoom, \zoom) rectangle (\zoom*2, \zoom*2);
        \draw[blue, thick] plot [domain=\zoom*0:\zoom*3] (\x,{1.5*\zoom - 2*\zoom*(\x-1.75*\zoom)});    
    \end{scope}

    % 
    \node[right, blue] at (\zoom*1.8,\zoom*1.5) {$\gamma_{\theta_{ij}}$};
    \node[right, domaincolor] at (\zoom*1.8,\zoom*2.5) {$\gamma$};
    
    % Mark a specific grid cell with a red square
    \draw[red, line width=0.4mm] (\zoom*1,\zoom*1) rectangle (\zoom*2,\zoom*2);
    \node[right] at (1.75,12) {$h$};
    % Approximation
  \end{scope}
\end{tikzpicture}

}



% Definitions
\def\edgeXcoord{2.3}
\def\velocity{0.4}
\newcommand{\functionA}[1]{((#1)^2/4+(#1)/3+2)}
% \newcommand{\functionB}[1]{(-((#1)-3.2)^2/3+1.1+2.4925)}
\newcommand{\functionB}[1]{(-((#1)-3.2)^2/3+1.1)}
\newcommand{\functionAbracket}[1]{{\functionA{#1}}}
\newcommand{\functionBbracket}[1]{{\functionB{#1}}}

% \newcommand{\functionATaylor}[1]{{(\functionA{1.5}-2*\functionA{0.5}+\functionA{-0.5})*(#1)-(\functionA{1.5}-2*\functionA{0.5}+\functionA{-0.5})*0.5+\functionA{0.5}}}
\newcommand{\functionATaylor}[1]{{\functionA{1.5}-\functionA{-0.5})/2*((#1)-0.5)+\functionA{0.5}}}

\newcommand{\PlotSubCellDiagramD}{
    % for colors https://latex-tutorial.com/color-latex/
            
    \begin{tikzpicture}[node distance=\whalf cm, scale=1, every node/.style={transform shape}]
    
        % The function
        \node at ((3, 3.2) {$\mathbf{\f(x)}$};
        \draw[ultra thick] plot [domain=-1:\edgeXcoord] (\x,\functionAbracket{\x});
        \draw[ultra thick] plot [domain=\edgeXcoord:4] (\x,\functionBbracket{\x});
                    
        % The function area
        \fill[fill=yellow!50] (-1, 0) -- plot [domain=-1:\edgeXcoord] (\x,\functionAbracket{\x}) -- (\edgeXcoord, 0) -- cycle;
        \fill[fill=yellow!50] (\edgeXcoord, 0) -- plot [domain=\edgeXcoord:4] (\x,\functionBbracket{\x}) -- (4, 0) -- cycle;
    
        % The cell limits
        \draw[ultra thick, dotted] (-1,0) -- (-1, \functionAbracket{-1});
        \draw[ultra thick, dotted] (0,0) -- (0, \functionAbracket{0});
        \draw[ultra thick, dotted] (1,0) -- (1, \functionAbracket{1});
        \draw[ultra thick, dotted] (2,0) -- (2, \functionAbracket{2});
        \draw[ultra thick, dotted] (3,0) -- (3, \functionBbracket{3});
        \draw[ultra thick, dotted] (4,0) -- (4, \functionBbracket{4});
        
        % The averages
        \node[MidnightBlue, opacity=1] at (0.5, 3.5) {Cell averages $\cellavg$};
        \draw[ultra thick, MidnightBlue, opacity=1] (-1,\functionAbracket{-0.5}) -- (0,\functionAbracket{-0.5});
        \draw[ultra thick, MidnightBlue, opacity=1] (0,\functionAbracket{0.5}) -- (1,\functionAbracket{0.5});
        \draw[ultra thick, MidnightBlue, opacity=1] (1,\functionAbracket{1.5}) -- (2,\functionAbracket{1.5});
        \newcommand{\average}{{\functionA{(2.0+\edgeXcoord)/2}*(\edgeXcoord-2)+\functionB{(\edgeXcoord+3.0)/2}*(3-\edgeXcoord)}}
        \draw[ultra thick, MidnightBlue, opacity=1] (2, \average) -- (3, \average);
        \draw[ultra thick, MidnightBlue, opacity=1] (3,\functionBbracket{3.5}) -- (4,\functionBbracket{3.5});
        
        % The edge
        \draw[thick, dashed, red, opacity=1] (\edgeXcoord,0) -- (\edgeXcoord, \functionAbracket{\edgeXcoord});
        \node[red, opacity=1] at (3.6, 2.5) {Dicontinuity};
        \node[red, opacity=1] at (\edgeXcoord, -0.5) {$X_0$};
        
        % velocity
        % \draw [arrow] (1-\velocity, 4) -- (1, 4);
        % \node [black, opacity=0] at (({1-\velocity)+\velocity/2}, 4.5) {$\Vec{v}$};
        
        % The flux
        % \fill[fill=green, opacity=0.25] (4-\velocity, 0) -- plot [domain=4-\velocity:4] (\x,\functionBbracket{\x}) -- (4, 0) -- cycle;
        % \draw[thick, green, ->] ({4-\velocity/2},-0.25) arc (200:340:{\velocity*3/4});
        % \fill[fill=green, opacity=0.25] (3-\velocity, 0) -- plot [domain=3-\velocity:3] (\x,\functionBbracket{\x}) -- (3, 0) -- cycle;
        % \draw[thick, green, ->] ({3-\velocity/2},-0.25) arc (200:340:{\velocity*3/4});
        % \fill[fill=green, opacity=0.25] (2-\velocity, 0) -- plot [domain=2-\velocity:2] (\x,\functionAbracket{\x}) -- (2, 0) -- cycle;
        % \draw[thick, green, ->] ({2-\velocity/2},-0.25) arc (200:340:{\velocity*3/4});
        % \fill[fill=green, opacity=0.25] (1-\velocity, 0) -- plot [domain=1-\velocity:1] (\x,\functionAbracket{\x}) -- (1, 0) -- cycle;
        % \draw[thick, green, ->] ({1-\velocity/2},-0.25) arc (200:340:{\velocity*3/4});
        % \draw[thick, green, ->] ({0-\velocity/2},-0.25) arc (200:340:{\velocity*3/4});
        % \node[green, opacity=0] at (2, -0.7) {Flux};
        
        % The stencil approximation
        \draw[ultra thin, dashed, ForestGreen, opacity=1] plot [domain=-1:2] (\x,\functionATaylor{\x});
        \draw[ultra thick, ForestGreen, opacity=1] plot [domain=0:1] (\x,\functionATaylor{\x});
        \node[ForestGreen, opacity=1] at (0, 2.7) {$P_i(x)$};

        % The stencil
        \node[MidnightBlue, opacity=1] at (-0.5, -0.5) {$\mathbf{i-1}$};
        \node[ForestGreen, opacity=1] at (0.5, -0.5) {$\mathbf{i}$};
        \node[MidnightBlue, opacity=1] at (1.5, -0.5) {$\mathbf{i+1}$};
        \node[MidnightBlue, opacity=1] at (3.5, -0.5) {$\mathbf{i+3}$};
    
    \end{tikzpicture}
}


% \begin{figure}
%     \centerline{    
%         \begin{tikzpicture}[node distance=\whalf cm, scale=1, every node/.style={transform shape}]
            
%             % Grid
%             \draw[step=1cm,gray, thin] (0,0) grid (3,3);
            
%             % Regions
%             \fill[yellow, opacity=0.25] plot [domain=0:3] (\x,{1.3+ 0.7*(\x-1.5) +(\x-1.5)^2/8}) -- (3,3) -- (0,3) -- cycle;
%             \fill[blue, opacity=0.25] plot [domain=0:3] (\x,{1.3+ 0.7*(\x-1.5) +(\x-1.5)^2/8}) -- (3,0) -- (0,0) -- cycle;
            
%             % Edge
%             \draw[red, thick] plot [domain=-0.5:3.5] (\x,{1.3+ 0.7*(\x-1.5) +(\x-1.5)^2/8});
%             % \node[red] at (-1.1, 1) {Discontinuity};
%             \node[red, rectangle, minimum width=2 cm, minimum height=0.5 cm, text centered, text width=3 cm] at (-0.25, 1.5) {Parametrized discontinuity};
            
%             % flux
%             \fill [fill=green!60!black, opacity=0.7, draw=black] (1.3,1) rectangle (2,2);
%             \draw[thick, green!60!black, ->] (1.6,1.7) arc (170:10:0.55);
%             \node[green!60!black, opacity=1] at (2, 2.5) {Flux};
            
%             % velocity
%             \draw [arrow] (1.3, 3.5) -- (2, 3.5);
%             \node [opacity=1] at (1.65,3.8) {$\Vec{v}$};
            
%             % Singular Cell
%             \draw [ultra thick, draw=blue!60, opacity=1] (1,1) rectangle (2,2);
%             \node[blue] at (1.5, 0.5) {Singular cell};
            
%             % Curve
%             % \draw[black, ultra thick, dashed] plot [domain=1:2] (\x,{1.35+ 0.7*(\x-1.5)});
%             % \node [black, rectangle, minimum width=1 cm, minimum height=0.25 cm, text centered, text width=0.5 cm] at (0.3, 1.5) {Fitted curve};
%             % \node[black] at (0, 1.5) {Fitted \\ curve};
            
%         \end{tikzpicture}
%     }
    
%     \caption{Diagram of subcell reconstruction in 2D}
%     \label{fig:subcell_schema2d}
% \end{figure}

